Adaptive Curriculum Generation from Demonstrations for Sim-to-Real Visuomotor Control

We propose Adaptive Curriculum Generation from Demonstrations (ACGD) for reinforcement learning in the presence of sparse rewards. Rather than designing shaped reward functions, ACGD adaptively sets the appropriate task difficulty for the learner by controlling where to sample from the demonstration trajectories and which set of simulation parameters to use. We show that training vision-based control policies in simulation while gradually increasing the difficulty of the task via ACGD improves the policy transfer to the real world. The degree of domain randomization is also gradually increased through the task difficulty. We demonstrate zero-shot transfer for two real-world manipulation tasks: pick-and-stow and block stacking. A video showing the results can be found at https://lmb.informatik.uni-freiburg.de/projects/curriculum/

==> algorithm.tex <==

\begin{algorithm}
\SetAlgorithmName{Algorithm}{algorithm}{list of algorithms name}
\SetAlgoLined
\SetKwFunction{FMain}{train\_policy}
    \SetKwProg{Fn}{Algorithm}{:}{}
    \Fn{\FMain}{
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Iterations $N$, initial policy $\pi_0$, interval $[\alpha, \beta]$, increment $\epsilon$}
\Output{final policy $\pi_{N}$}    
\nl$sr_d, sr_r,\delta_d,\delta_r \leftarrow 0$\;
\nl    \For{$i\leftarrow 1$ \KwTo $N$}{
\nl        $ rollouts \leftarrow \texttt{generate\_rollouts()}$\;
\nl        $ \pi_i \leftarrow \texttt{update\_policy}(rollouts, \pi_{i-1})$\;
\nl        update success rate $sr_d$\;
\nl        update success rate $sr_r$\;
            \BlankLine
            \tcc{update difficulty parameters}
% \nl        \uIf{$sr_d > \beta$}{
% \nl            $\delta_d \leftarrow $clip$(\delta_d + \epsilon, 0, 1)$\;
%             }
% \nl        \uElseIf{$sr_d < \alpha$}{
% \nl            $\delta_d \leftarrow $clip$(\delta_d - \epsilon, 0, 1)$\;
%             }
%             \BlankLine
% \nl        \uIf{$sr_r > \beta$}{
% \nl            $\delta_r \leftarrow $clip$(\delta_r + \epsilon, 0, 1)$\;
%             }
% \nl         \uElseIf{$sr_r < \alpha$}{
% \nl            $\delta_r \leftarrow $clip$(\delta_r - \epsilon, 0, 1)$\;
        % }
\nl$\delta_d^{(i+1)}=
    \begin{cases}
      \delta_d^{(i)} + \epsilon, & \text{if}\ sr_d >\beta \\
      \delta_d^{(i)} - \epsilon, & \text{if}\ sr_d <\alpha \\
      \delta_d^{(i)}, & \text{otherwise}
    \end{cases}$\;
    \BlankLine
\nl$\delta_r^{(i+1)}=
    \begin{cases}
      \delta_r^{(i)} + \epsilon, & \text{if}\ sr_r >\beta \\
      \delta_r^{(i)} - \epsilon, & \text{if}\ sr_r <\alpha \\
      \delta_r^{(i)}, & \text{otherwise}
    \end{cases}$
    }
}
\setcounter{AlgoLine}{0}
\BlankLine
\BlankLine
\SetKwFunction{FMain}{generate\_rollouts}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain}{
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{Batchsize $B$, policy $\pi_i$, success rate $sr_r$, training progress $prog$, difficulty $\delta_d$, difficulty $\delta_r$, demonstrations $\mathcal{D}$, episode length $T$, window size $\sigma$, env params $\mathcal{H}$}
\nl    $rollouts \leftarrow []$\;
\nl    \For{$j\leftarrow 0$ \KwTo $B$}{
\nl        sample action $a_j \sim \pi_i$\;
% \nl        $o, r, done \leftarrow env.\texttt{step}(a)$\;
\nl         execute action $a_j$ and receive state $s_{j+1}$, observation $o_j$ and reward $r_j$\;
\nl        $rollouts.\texttt{append}([s_{j+1}, o_j, r_j])$\;
\SetKwProg{With}{with}{ do}{}
\SetKwProg{Other}{otherwise}{}{}
\nl        \uIf{terminal $s$}{
\nl            \With{probability $p=0.5 (sr_r + prog)$}{
\tcc{reset from demonstrations}
% \nl                $env.\texttt{set\_difficulty}(\delta_d)$\;
\nl                 for each parameter $h \in \mathcal{H}$ : set $h \leftarrow \delta_d $\;
\nl                sample demonstration $d \sim D$\;
\nl                sample timestep $t \sim $ unif$((1 - \delta_d) T - \sigma, (1 - \delta_d)T + \sigma)$\;
% \nl                $env.\texttt{reset\_from\_demonstration}(d_t)$\;
\nl                set start state to demonstration: $s_{j+1} \leftarrow d_t$ 
            }
\nl            \Other{}{
\tcc{regular reset}
\nl                 for each parameter $h \in \mathcal{H}$ : set $h \leftarrow \delta_r $\;
\nl                sample start state from start state distribution: $s_{j+1} \sim \rho_0$\;
            }
        }
    }
    \textbf{return} $rollouts$\;
}
\caption{Adaptive Curriculum Generation from Demonstrations}
\label{alg1}
\end{algorithm}
